Rasterized Edge Gradients: Handling Discontinuities Differentiably

Computing the gradients of a rendering process is paramount for diverse applications in computer vision and graphics. However, accurate computation of these gradients is challenging due to discontinuities and rendering approximations, particularly for surface-based representations and rasterization-based rendering. We present a novel method for computing gradients at visibility discontinuities for rasterization-based differentiable renderers. Our method elegantly simplifies the traditionally complex problem through a carefully designed approximation strategy, allowing for a straightforward, effective, and performant solution. We introduce a novel concept of micro-edges, which allows us to treat the rasterized images as outcomes of a differentiable, continuous process aligned with the inherently non-differentiable, discrete-pixel rasterization. This technique eliminates the necessity for rendering approximations or other modifications to the forward pass, preserving the integrity of the rendered image, which makes it applicable to rasterized masks, depth, and normals images where filtering is prohibitive. Utilizing micro-edges simplifies gradient interpretation at discontinuities and enables handling of geometry intersections, offering an advantage over the prior art. We showcase our method in dynamic human head scene reconstruction, demonstrating effective handling of camera images and segmentation masks.

==> sec/2_related_work_orig.tex <==
\section{Related work}
\label{sec:related_work}

Differentiable rendering is one of the key building blocks for many existing computer vision problems, such as 3d object reconstruction~\cite{kato2018neural,yan2016perspective,tulsiani2017multi,yang2018learning,choy20163d}, 3d object prediction~\cite{chen2019learning,beker2020monocular,chen2021dib,henzler2021unsupervised}, pose estimation~\cite{pavlakos2018learning,bogo2016keep,ge20193d,baek2019pushing} novel view synthesis~\cite{mildenhall2021nerf,barron2021mip,zhang2020nerf++,muller2022instant,kerbl20233d}, as well as newly emerging applications such as text-to-3D generative models~\cite{poole2022dreamfusion,lin2023magic3d,tsalicoglou2023textmesh,shi2023mvdream}.
%
%\subsection{Overview}
%\label{subsec:overview}
%
Differentiable rendering employs a wide array of underlying 3D representations. These include explicit surfaces like mesh-based representations~\cite{loper2014opendr,deLaGorce:2011:MHP:2006854.2007005,laine2020modular}, implicit surfaces~\cite{park2019deepsdf,jiang2020sdfdiff,vicini2022differentiable,bangaru2022differentiable}, point clouds~\cite{roveri2018pointpronets,wiles2020synsin,kerbl20233d}, explicit or implicit volume representations~\cite{yan2016perspective,lombardi2019neural,liu2020neural,yu2021plenoxels,mildenhall2021nerf,niemeyer2020differentiable,barron2021mip}, and hybrid representations~\cite{chan2022efficient,muller2022instant}.
There is also a body of work on extracting explicit representations from implicit or volumetric ones, e.g.\ distilling meshes from NeRF~\cite{hedman2021baking,chen2023mobilenerf}.
%
%In the following, we focus on methods that render meshes and also handle discontinuities at occlusion boundaries.
For a comprehensive introduction to differentiable rendering, we refer the reader to Zhao {\em et al.}'s excellent SIGGRAPH course notes~\cite{Zhao2020DifferentiableCourse}.

As highlighted in our introduction in \S\ref{sec:intro}, mesh optimization is often more challenging compared to implicit and volumetric methods, leading to the latter's dominance in the field as noted by Roessle {\em et al.}~\cite{roessle2022dense}.
However, meshes offer advantages in high-performance rendering, especially when accelerated with hardware rasterizers, and additionally often also imply a registration when using a predefined topology.
% Our work is centered on developing high-performance differentiable rendering methods that are efficient both in testing and training phases.
%
Rendering methods for meshes generally fall into two primary categories: rasterization-based (\S\ref{subsec:rasterization}) and ray tracing-based (\S\ref{subsec:raytracing}).
Differentiable ray tracing approaches often employ physically-based rendering with Monte Carlo path tracing, as seen in a versatile framework Mitsuba 3~\cite{NimierDavidVicini2019Mitsuba2,Jakob2020DrJit}.
% Such frameworks focus on global illumination, physics-based materials, media, etc.
Despite their flexibility, the computational expense of such ray tracing frameworks restrict their practicality in optimization-intensive tasks~\cite{laine2020modular}.

Our work focuses on high-performance methods that can render high-resolution images and backpropagate through the rendering process in milliseconds to make optimizations that require millions of iterations practically feasible.
This is particularly vital for reconstructing high-quality, dynamic scenes, like facial performance capture, where alternative representations would be prohibitively expensive.

\subsection{Rasterization}
\label{subsec:rasterization}

Regardless of the particular rendering method, handling meshes in differentiable rendering pipelines is not easy because the pixel values depend on visibility terms that are not differentiable at objects boundaries.
%
%Differentiability at boundaries is handled quite differently by ray-tracing and rasterization-based methods.
Differentiable ray tracing frameworks attempt to compute boundary integral and visibility gradients that will converge to the correct result with a growing number of Monte Carlo samples.
However, similar properties are not found in rasterization methods, primarily because boundary sampling or parametrizing sample locations is not feasible with fixed-grid rasterization and z-buffer based rendering.
%
Consequently, there are primarily two types of solutions for rasterization based differentiable rendering: 1) approximating the derivatives while maintaining that the rendering model remains unchanged; 2) approximating the rendering model with an inherently differentiable formulation.

\textbf{Approximating derivatives.}
% Explicit boundary / Dirac delta integration
The pioneering work of de La Gorce {\em et al.}~\cite{deLaGorce:2011:MHP:2006854.2007005} approached hand mesh fitting through inverse rendering, splitting the rendering integral into two distinct components: a continuous region amenable to direct application of the chain rule, and the occlusion boundaries.
Within their DEODR framework, they introduced the concept of 'occlusion forces,' which represent the variations in the objective function along line segments aligned with triangle edges at occlusion boundaries.
Loper {\em et al.}\cite{loper2014opendr}, in their OpenDR framework, proposed a simplification by identifying discontinuities post-rasterization and approximating the boundary term using differential filters, such as the Sobel filter.
Although the method by de La Gorce {\em et al.} aligns more closely with an analytical solution compared to the more approximate approach of Loper et al., it does present drawbacks.
Primarily, the former method is marked by its complexity and the necessity to interact with the source geometry for detecting visibility discontinuities.

The method introduced by Laine {\em et al.}~\cite{laine2020modular} in their 'Nvdiffrast' framework deserves separate mention.
This approach addresses the challenges posed by point-sampled visibility, which not only causes aliasing at visibility discontinuities but also fails to produce visibility-related gradients.
The novel aspect of this method is its post-rasterization differentiable analytic antialiasing step, which transforms sharp discontinuities into smooth transitions, enabling gradient computation.
This technique builds upon the concepts established by de La Gorce {\em et al.} and adapts a common real-time graphics antialiasing approach, reminiscent of techniques like FXAA.
%
Analytical antialiasing in this method is achieved by estimating coverage, although this estimate is only exact for vertical and horizontal edges.
A significant limitation is that it retains information about only one triangle per pixel.
Consequently, if triangles containing silhouette edges do not overlap with the pixel center, they will be overlooked during the antialiasing process, and the boundary will miss the discontinuity gradients.
Moreover, analytical antialiasing alters the rasterized image and is inherently approximate, and as a result the obtained gradients at discontinuities are also approximate.
We will delve further into this behavior in the Analysis section (\S\ref{sec:analysis}).
Regrettably, the analytical antialiasing method also remains quite complex.
It necessitates the maintenance of a specialized data structure to retrieve connectivity information, typically implemented using a hashmap.
Additionally, it involves projecting vertices into pixel space and executing intricate gradient computations based on the geometric coverage of the pixel by the primitive.

\textbf{Approximating rendering.}
Rhodin {\em et al.}~\cite{rhodin2015versatile}  introduced a method to mitigate discontinuities at object boundaries by rendering these as fuzzy edges, thereby gradually transitioning the object to transparency as it approaches its boundaries.
Building on this concept, Liu {\em et al.}~\cite{liu2019softras} advanced the approach with the development of the 'Soft Rasterizer.' This technique not only blurs the object boundaries but also implements a weighted average calculation of the primitives in the depth dimension.
This approach ensures that gradients are propagated even to occluded primitives, thereby allowing for optimization of the primitives' positioning in the depth dimension.
Unfortunately, the 'Soft Rasterizer' method is significantly slowed down by hidden geometry and becomes extremely expensive with larger number of primitives, as noted by Laine {\em et al.}~\cite{laine2020modular}.
For our method we try to avoid changing the rendering model.
In fact, our technique avoids any modifications of the rasterized image altogether.

\subsection{Raytracing.}
\label{subsec:raytracing}

Differentiable ray tracing methods, whether focused on direct illumination or employing physically based rendering with path tracing, tend to target a more computationally expensive operational regime and adopt a more principled approach.
The pixel color is the result of integrating all light paths that intersect the pixel filter.
Consequently, while the integrand may be discontinuous, the integral itself remains continuous and, therefore, differentiable.

Recent advancements~\cite{Li:2018:DMC,Zhang2019DTRT} have decomposed the gradient of such integrals into two components: the integral over discontinuities containing Dirac delta functions, and the integral over the derivative of the continuous part, computable via automatic differentiation.
%
Li {\em et al.}~\cite{Li:2018:DMC} achieved this by replacing integration over Dirac deltas with integration along discontinuity boundaries, associated with triangle edges.
Alternatively, Zhang {\em et al.}\cite{Zhang2019DTRT} utilized Reynold's transport theorem, an extension of Leibniz's rule for multidimensional integrals, to achieve a similar two-term decomposition.
However, these methods are complex and require identifying and sampling the discontinuities, including boundaries, silhouettes, and occlusions.
Li {\em et al.} call this ``edge sampling'' and focus on triangle edges.

Loubet {\em et al.}~\cite{Loubet2019Reparameterizing}  tackle the challenge of sampling discontinuity boundaries by using a change of variables that removes the discontinuity
of the integrand, which can be handled using the chain rule if such a transformation exists.
However, finding such a transformation is complex, particularly for intricate geometries.
They suggest dividing the integral into smaller segments, each precisely represented by a spherical rotation to capture discontinuities.
Building on this, Bangaru {\em et al.}\cite{bangaru2020unbiased} enhance the approach by using warped area fields instead of spherical rotations, addressing the bias in Loubet {\em et al.}'s method.
Despite the elegance of these methods, their robust practical application remains a significant challenge.


\subsection{Relation to Prior Art}
\label{subsec:prior_art}

In this work, we deliberately bypass physically based rendering, global illumination, and lighting/material models, and instead focus exclusively on rasterization-based approaches for their speed.
%
We draw inspiration from state-of-the-art differentiable ray tracing techniques, adapting these insights for differentiable rasterizers.
We attempt to take the core idea of the edge sampling method~\cite{Li:2018:DMC} and analytical antialiasing and distill this into a much simpler yet effective method that also provides accurate gradients.
%
Our method shares some features with prior approximate gradient techniques, but we identify the sources of our approximations and accurately devise a discretization scheme within the rasterized pixel grid.
%
Notably, our method's simplicity allows handling self-penetrating geometry, an issue not addressed in previous research.
Although interpenetrating triangles frequently arise in optimization processes, resolving this through geometry intersection detection and edge extraction is complex, computationally demanding, and not feasible at every optimization step.

%
%Importantly, none of the above approaches handle the case of interpenetrating triangles. Two subtle yet important details are (1) how discontinuities are detected, and (2) how the continuous image function is extended for computing the boundary terms. The above methods~\cite{deLaGorce:2011:MHP:2006854.2007005,Li:2018:DMC,Zhang2019DTRT} explicitly only consider triangle edges and therefore miss all discontinuities due to interpenetrating triangles.


%For our discussion, it will suffice to think of a pixel as a sensor that integrates light over its surface, and
%conceptualize the value of a rendered pixel as the integral of an image function $i(\boldsymbol{\theta}, \mathbf{x})$
%over the pixel area, i.e.,
%$\int_{\Omega} i(\boldsymbol{\theta}, \mathbf{x}) \mathbf{d}\mathbf{x}$, where $\mathbf{x}{\in} \Omega$ is the domain of pixel coordinates and $\boldsymbol{\theta}$ define rendering parameters.
%%We are interested in computing the change of this integral for infinitesimal changes in the parameters $\boldsymbol{\theta}$.
%
%
%Recent work~\cite{Li:2018:DMC,Zhang2019DTRT} has derived a more general but equivalent decomposition of the gradient into two terms,
%
%\begin{equation}
%\frac{\partial}{\partial \boldsymbol{\theta}} \int_{\Omega} {i}(\boldsymbol{\theta}, \mathbf{x}) \mathbf{dx} = \int_{\Omega \setminus D} \frac{\partial}{\partial \boldsymbol{\theta}} {i}(\boldsymbol{\theta}, \mathbf{x}) \mathbf{dx} + I_D.
%\label{eq:pixel_rendering}
%\end{equation}

